Bitvector-aware Query Optimization for Decision Support Queries (extended version)

Bitvector filtering is an important query processing technique that can significantly reduce the cost of execution, especially for complex decision support queries with multiple joins. Despite its wide application, however, its implication to query optimization is not well understood. In this work, we study how bitvector filters impact query optimization. We show that incorporating bitvector filters into query optimization straightforwardly can increase the plan space complexity by an exponential factor in the number of relations in the query. We analyze the plans with bitvector filters for star and snowflake queries in the plan space of right deep trees without cross products. Surprisingly, with some simplifying assumptions, we prove that, the plan of the minimal cost with bitvector filters can be found from a linear number of plans in the number of relations in the query. This greatly reduces the plan space complexity for such queries from exponential to linear. Motivated by our analysis, we propose an algorithm that accounts for the impact of bitvector filters in query optimization. Our algorithm optimizes the join order for an arbitrary decision support query by choosing from a linear number of candidate plans in the number of relations in the query. We implement our algorithm in Microsoft SQL Server as a transformation rule. Our evaluation on both industry standard benchmarks and customer workload shows that, compared with the original Microsoft SQL Server, our technique reduces the total CPU execution time by 22%-64% for the workloads, with up to two orders of magnitude reduction in CPU execution time for individual queries.

==> algorithm_extract_snowflake.tex <==
\begin{algorithm}
\DontPrintSemicolon
\SetAlgoLined
\LinesNumbered

\caption{\changed{Extract a snowflake from a join graph}}
\label{algorithm:extract_snowflake}

\SetKwProg{FuncExtractSnowflake}{}{:}{}
\FuncExtractSnowflake{\textbf{ExtractSnowflake($G$)}}{
	\KwIn{Join graph $G$}
	\KwOut{Snowflake $G'$}
%	\tcc{Fact table is the right most leaf}
	$n \leftarrow 0$\;
	$G_{sorted} \leftarrow SortByCardinalityAsc(G)$\;
	\ForEach{$g$ in $G_{sorted}$}{
		\If{$g$ is an unoptimized fact table}{
			\If{$n == 0$}{
				$G' \leftarrow ExpandSnowflake(g)$
			}
			$n \leftarrow n + 1$
		}
	}
	\lIf{$n == 1$}{
		$G'\leftarrow G$
	}
	\Return{$G'$}
}

\end{algorithm}

==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

\paragraph{We implement on a commercial database}
\paragraph{DBMS has bitmap optimization for QE}
\paragraph{The DBMS has a macro module to detect snowflake patterns}
\paragraph{Snowflakes are detected recursively}
\paragraph{Additional rules are applied before and after the snowflake patterns}
\paragraph{The plan is picked or not is subjective to the cost model and cardinality estimation}


==> infeasibility.tex <==
\section{Infeasibility Results on DP-based Query Optimization}
\label{sec:infeasibility}

\todo{Remove this section}

While the bitmaps are straightforward runtime optimizations, they are either incorporated into the query plan as an after-thought where the query optimizer neglects the bitmaps during its plan search or they are infused into various rule-based heuristics in a commercial query optimizer.

While it seems that the bitmaps are not considered holistically during query optimization is just a compromise of engineering complicated legacy code base, we have dived into this problem and discovered a fact that is far more striking.

Most of the current query optimization frameworks, either bottom up or top town, are essentially based on dynamic programming. Surprisingly, a dynamic programming based query optimization framework is fundamentally infeasible to incorporate bitmaps into its plan search because the plan search algorithm does not satisfy the property of optimal substructures anymore with bitmaps.


\todo{An example of why optimal substructures are not satisfied with bitmaps}
\begin{theorem}
	\textbf{Substructure optimality violation with bitmap filters: }
	The substructure optimality of the existing top-down or bottom-up DP-based query optimization framework is violated by bitmap filters.
\end{theorem}

\todo{Refer to the example in the introduction}

\todo{Intuitively, outline the issue in satisfying the optimal substructures: where to push down}

\begin{theorem}
	\textbf{Exponential increase of substructures in DP: }
	Let $q$ be a query of $n$ relations. Let $m_1$ and $m_2$ be the number of optimal substructures needed to for a top-down or bottom-down DP-based query optimization framework with and without bitmap filters.
	Then there exists a query $q$ such that $m_2>a^n\cdot m_1$, where $a$ is a constant and $a>1$.
\end{theorem}

\begin{figure}
	\begin{subfigure}[b]{.22\textwidth}
		\centering
		\includegraphics[width=.9\linewidth]{./figures/dp_query}
		\caption{A join graph of $2n+1$ relations with many-to-many join conditions}
		\label{fig:dp:query}
	\end{subfigure}
	\quad
	\begin{subfigure}[b]{.23\textwidth}
		\centering
		\includegraphics[width=.9\linewidth]{./figures/dp_plan}
		\caption{A subplan space results in $n!$ substructures with bitmap filters}
		\label{fig:dp:plan}
	\end{subfigure}
	\caption{Example of increasing the substructures by more than an exponential factor with bitmap filters in DP-based query optimization framework}
	\label{fig:dp}
\end{figure}

\begin{proof}
We show an example where the number of substructures of a DP-based query optimization framework increases by more than exponential factor with bitmap filters.

Figure~\ref{fig:dp:query} shows the join graph of a query of $2n+1$ relations, where each edge is a many-to-many join of two relations. Consider the plan search space of right deep tree with cross products, we want to analyze the number of subplans that need to be kept for DP-based query optimization with and without bitmap filters.

Without bitmap filters, the DP algorithm keeps the optimal subplans of joining $k$ relations out of $2n+1$ relations. Thus, the total number of subplans kept is $m_1=\sum_{i=1}^(2n+1)\binom{2n+1}{i}=2^(2n+1)$.

Now consider the optimal subplans with bitmap filters. Consider a particular plan structure as shown in Figure~\ref{fig:dp:plan}, where $R_0$ is the right most leaf, and $X_1, X_2,\cdots, X_n$ is a permutation of $R_{1,2}, R_{2,2}, \cdots, R_{n, 2}$. Since $R_{i, 1}$ joins with both $R_0$ and $R_{i,2}$, the bitmap filter created from $R_{i, 1}$ will be pushed down to the right most join result that contains both $R_0$ and $R_{i,2}$. Thus, every permutation of $R_{1, 2}, R_{2, 2}, \cdots, R_{n, 2}$ corresponds to a different sequence of how bitmap filters from $Y_1, Y_2, \cdots, Y_n$ apply to the join results. Thus, the total number of subplans that need to be kept for $T(X_1,X_2, \cdots, X_n, R_0)$ is $n!$, and $m_2>n!$.

Because $\lim_{n\to\infty}\frac{n!}{c^n}=\infty$ for any constant $c$, with large enough $n$, we have $\frac{n!}{2^{2n+1}}\geq \frac{n!}{2\cdot 4^{n}}=\frac{a^n}{2}\cdot \frac{n!}{(4a)^{n}}\geq \frac{a^n}{2}$, where $a>1$ is a constant.

Thus, $m_2>a^n\cdot m_1$.

\end{proof}


==> reference.tex <==
@inproceedings{bqo20sigmod,
	title={Bitvector-aware query optimization for decision support queries},
	author={Ding, Bailu, and Chaudhuri, Surajit, and Narasayya, Vivek},
	booktitle = {Proceedings of the 2020 ACM SIGMOD International Conference on Management of Data},
	year={2020},
}

@article{almeida2007scalable,
	title={Scalable bloom filters},
	author={Almeida, Paulo S{\'e}rgio and Baquero, Carlos and Pregui{\c{c}}a, Nuno and Hutchison, David},
	journal={Information Processing Letters},
	volume={101},
	number={6},
	pages={255--261},
	year={2007},
	publisher={Elsevier}
}

@inproceedings{putze2007cache,
	title={Cache-, hash-and space-efficient bloom filters},
	author={Putze, Felix and Sanders, Peter and Singler, Johannes},
	booktitle={International Workshop on Experimental and Efficient Algorithms},
	pages={108--121},
	year={2007},
	organization={Springer}
}

@inproceedings{lang2019performance,
  author    = {Harald Lang and
Thomas Neumann and
Alfons Kemper and
Peter A. Boncz},
title     = {Performance-Optimal Filtering: Bloom overtakes Cuckoo at High-Throughput},
journal   = {{PVLDB}},
volume    = {12},
number    = {5},
pages     = {502--515},
year      = {2019},
doi       = {10.14778/3303753.3303757},
timestamp = {Mon, 04 Nov 2019 15:39:16 +0100},
biburl    = {https://dblp.org/rec/bib/journals/pvldb/LangNKB19},
bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{neumann2009query,
author = {Neumann, Thomas},
title = {Query Simplification: Graceful Degradation for Join-Order Optimization},
year = {2009},
isbn = {9781605585512},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1559845.1559889},
doi = {10.1145/1559845.1559889},
booktitle = {Proceedings of the 2009 ACM SIGMOD International Conference on Management of Data},
pages = {403--414},
numpages = {12},
keywords = {query optimization, hypergraphs, complex joins},
location = {Providence, Rhode Island, USA},
series = {SIGMOD'09}
}


@inproceedings{graefe1993query,
author = {Graefe, Goetz},
title = {Query Evaluation Techniques for Large Databases},
year = {1993},
issue_date = {June 1993},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {25},
number = {2},
issn = {0360-0300},
url = {https://doi.org/10.1145/152610.152611},
doi = {10.1145/152610.152611},
journal = {ACM Comput. Surv.},
month = jun,
pages = {73--169},
numpages = {97},
keywords = {object-oriented database systems, set-matching algorithms, operator model of parallelization, complex query evaluation plans, parallel algorithms, iterators, dynamic query evaluation plans, sort-hash duality, extensible database systems, relational database systems}
}

@inproceedings{neumann2013taking,
  author    = {Thomas Neumann and
C{\'{e}}sar A. Galindo{-}Legaria},
title     = {Taking the Edge off Cardinality Estimation Errors using Incremental
Execution},
booktitle = {Datenbanksysteme f{\"{u}}r Business, Technologie und Web (BTW),
15. Fachtagung des GI-Fachbereichs "Datenbanken und Informationssysteme"
(DBIS), 11.-15.3.2013 in Magdeburg, Germany. Proceedings},
series    = {{LNI}},
volume    = {{P-214}},
pages     = {73--92},
publisher = {{GI}},
year      = {2013},
url       = {https://dl.gi.de/20.500.12116/17356},
timestamp = {Mon, 18 Nov 2019 15:06:18 +0100},
biburl    = {https://dblp.org/rec/bib/conf/btw/0001G13},
bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{leis2018query,
  author    = {Viktor Leis and
Bernhard Radke and
Andrey Gubichev and
Atanas Mirchev and
Peter A. Boncz and
Alfons Kemper and
Thomas Neumann},
title     = {Query optimization through the looking glass, and what we found running
the Join Order Benchmark},
journal   = {{VLDB} J.},
volume    = {27},
number    = {5},
pages     = {643--668},
year      = {2018},
url       = {https://doi.org/10.1007/s00778-017-0480-7},
doi       = {10.1007/s00778-017-0480-7},
timestamp = {Wed, 10 Oct 2018 15:21:17 +0200},
biburl    = {https://dblp.org/rec/bib/journals/vldb/LeisRGMBKN18},
bibsource = {dblp computer science bibliography, https://dblp.org}
}

@online{tpcds,
	title = {{TPC-DS}},
	url= {http://www.tpc.org/tpcds/},
	year={2012},
}

@inproceedings{galindo2008optimizing,
author={C. A. {Galindo-Legaria} and T. {Grabs} and S. {Gukal} and S. {Herbert} and A. {Surna} and S. {Wang} and W. {Yu} and P. {Zabback} and S. {Zhang}},
booktitle={2008 IEEE 24th International Conference on Data Engineering},
title={Optimizing Star Join Queries for Data Warehousing in Microsoft SQL Server},
year={2008},
volume={},
number={},
pages={1190-1199},
keywords={data warehouses;decision support systems;pattern matching;query processing;relational databases;SQL;star join query;data warehousing;microsoft SQL server;mainstream data warehouses;multiterabyte range;decision support query;database query processors;query optimization;relational data warehouses;pattern matching;star query patterns;selectivity query;bitmap filters;Warehousing;Data warehouses;Pattern matching;Filters;Transaction databases;Relational databases;Query processing;Shape;Companies;Business},
doi={10.1109/ICDE.2008.4497528},
ISSN={2375-026X},
month={April},}

@inproceedings{bernstein1981using,
author = {Bernstein, Philip A. and Chiu, Dah-Ming W.},
title = {Using Semi-Joins to Solve Relational Queries},
year = {1981},
issue_date = {January 1981},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {28},
number = {1},
issn = {0004-5411},
url = {https://doi.org/10.1145/322234.322238},
doi = {10.1145/322234.322238},
journal = {J. ACM},
month = jan,
pages = {25--40},
numpages = {16}
}


@inproceedings{Weininger:2002:EEJ:564691.564754,
author = {Weininger, Andreas},
title = {Efficient Execution of Joins in a Star Schema},
year = {2002},
isbn = {1581134975},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/564691.564754},
doi = {10.1145/564691.564754},
booktitle = {Proceedings of the 2002 ACM SIGMOD International Conference on Management of Data},
pages = {542--545},
numpages = {4},
location = {Madison, Wisconsin},
series = {SIGMOD'02}
}


@inproceedings{Karayannidis:2002:PSQ:1287369.1287432,
  author    = {Nikos Karayannidis and
Aris Tsois and
Timos K. Sellis and
Roland Pieringer and
Volker Markl and
Frank Ramsak and
Robert Fenk and
Klaus Elhardt and
Rudolf Bayer},
title     = {Processing Star Queries on Hierarchically-Clustered Fact Tables},
booktitle = {Proceedings of 28th International Conference on Very Large Data Bases,
{VLDB} 2002, Hong Kong, August 20-23, 2002},
pages     = {730--741},
publisher = {Morgan Kaufmann},
year      = {2002},
doi       = {10.1016/B978-155860869-6/50070-6},
timestamp = {Thu, 06 Jun 2019 13:25:09 +0200},
biburl    = {https://dblp.org/rec/bib/conf/vldb/KarayannidisTSPMRFEB02},
bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Das:2015:QOO:2824032.2824074,
  author    = {Dinesh Das and
Jiaqi Yan and
Mohamed Za{\"{\i}}t and
Satyanarayana R. Valluri and
Nirav Vyas and
Ramarajan Krishnamachari and
Prashant Gaharwar and
Jesse Kamp and
Niloy Mukherjee},
title     = {Query Optimization in Oracle 12c Database In-Memory},
journal   = {{PVLDB}},
volume    = {8},
number    = {12},
pages     = {1770--1781},
year      = {2015},
doi       = {10.14778/2824032.2824074},
timestamp = {Thu, 16 Aug 2018 11:33:42 +0200},
biburl    = {https://dblp.org/rec/bib/journals/pvldb/DasYZVVKGKM15},
bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Hsiao:1994:PEM:191839.191879,
author = {Hsiao, Hui-I and Chen, Ming-Syan and Yu, Philip S.},
title = {On Parallel Execution of Multiple Pipelined Hash Joins},
year = {1994},
isbn = {0897916395},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/191839.191879},
doi = {10.1145/191839.191879},
booktitle = {Proceedings of the 1994 ACM SIGMOD International Conference on Management of Data},
pages = {185--196},
numpages = {12},
location = {Minneapolis, Minnesota, USA},
series = {SIGMOD'94}
}

@inproceedings{bloom1970space,
author = {Bloom, Burton H.},
title = {Space/Time Trade-Offs in Hash Coding with Allowable Errors},
year = {1970},
issue_date = {July 1970},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {13},
number = {7},
issn = {0001-0782},
url = {https://doi.org/10.1145/362686.362692},
doi = {10.1145/362686.362692},
journal = {Commun. ACM},
month = jul,
pages = {422--426},
numpages = {5},
keywords = {retrieval efficiency, hash addressing, storage layout, searching, storage efficiency, retrieval trade-offs, scatter storage, hash coding}
}

@inproceedings{bratbergsengen1984hashzng,
author    = {Kjell Bratbergsengen},
title     = {Hashing Methods and Relational Algebra Operations},
booktitle = {Tenth International Conference on Very Large Data Bases, August 27-31,
1984, Singapore, Proceedings},
pages     = {323--333},
publisher = {Morgan Kaufmann},
year      = {1984},
timestamp = {Wed, 29 Mar 2017 16:45:24 +0200},
biburl    = {https://dblp.org/rec/bib/conf/vldb/Bratbergsengen84},
bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{valduriez1984join,
author = {Valduriez, Patrick and Gardarin, Georges},
title = {Join and Semijoin Algorithms for a Multiprocessor Database Machine},
year = {1984},
issue_date = {March 1984},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {9},
number = {1},
issn = {0362-5915},
url = {https://doi.org/10.1145/348.318590},
doi = {10.1145/348.318590},
journal = {ACM Trans. Database Syst.},
month = mar,
pages = {133--161},
numpages = {29}
}


@inproceedings{chen1993applying,
  author    = {Ming{-}Syan Chen and
Hui{-}I Hsiao and
Philip S. Yu},
title     = {Applying Hash Filters to Improving the Execution of Bushy Trees},
booktitle = {19th International Conference on Very Large Data Bases, August 24-27,
1993, Dublin, Ireland, Proceedings},
pages     = {505--516},
publisher = {Morgan Kaufmann},
year      = {1993},
timestamp = {Tue, 07 Nov 2017 16:24:37 +0100},
biburl    = {https://dblp.org/rec/bib/conf/vldb/VhanHY93},
bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{chen1997applying,
  author    = {Ming{-}Syan Chen and
Hui{-}I Hsiao and
Philip S. Yu},
title     = {On Applying Hash Filters to Improving the Execution of Multi-Join
Queries},
journal   = {{VLDB} J.},
volume    = {6},
number    = {2},
pages     = {121--131},
year      = {1997},
url       = {https://doi.org/10.1007/s007780050036},
doi       = {10.1007/s007780050036},
timestamp = {Sun, 28 May 2017 13:19:16 +0200},
biburl    = {https://dblp.org/rec/bib/journals/vldb/ChenHY97},
bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{chen1992interleaving,
author={M. -. {Chen} and P. S. {Yu}},
journal={IEEE Transactions on Parallel and Distributed Systems},
title={Interleaving a join sequence with semijoins in distributed query processing},
year={1992},
volume={3},
number={5},
pages={611--621},
keywords={database theory;distributed databases;query processing;relational databases;distributed query processing;interleaving;beneficial semijoins;join sequence tree;reducible relations;Interleaved codes;Query processing;Data communication;Tree graphs;Marine vehicles;Relational databases;Computer networks;Context;Cost function},
doi={10.1109/71.159044},
ISSN={2161-9883},
month={Sep.},}

@inproceedings{seshadri1996cost,
author = {Seshadri, Praveen and Hellerstein, Joseph M. and Pirahesh, Hamid and Leung, T. Y. Cliff and Ramakrishnan, Raghu and Srivastava, Divesh and Stuckey, Peter J. and Sudarshan, S.},
title = {Cost-Based Optimization for Magic: Algebra and Implementation},
year = {1996},
isbn = {0897917944},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/233269.233360},
doi = {10.1145/233269.233360},
booktitle = {Proceedings of the 1996 ACM SIGMOD International Conference on Management of Data},
pages = {435--446},
numpages = {12},
location = {Montreal, Quebec, Canada},
series = {SIGMOD'96}
}

@inproceedings{beeri1991power,
	title={On the power of magic},
	author={Beeri, Catriel and Ramakrishnan, Raghu},
	journal={The journal of logic programming},
	volume={10},
	number={3-4},
	pages={255--299},
	year={1991},
	publisher={Elsevier}
}

@inproceedings{chan1998bitvector,
author = {Chan, Chee-Yong and Ioannidis, Yannis E.},
title = {Bitmap Index Design and Evaluation},
year = {1998},
isbn = {0897919955},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/276304.276336},
doi = {10.1145/276304.276336},
booktitle = {Proceedings of the 1998 ACM SIGMOD International Conference on Management of Data},
pages = {355--366},
numpages = {12},
location = {Seattle, Washington, USA},
series = {SIGMOD'98}
}

@inproceedings{lahiri2015oracle,
author={T. {Lahiri} and S. {Chavan} and M. {Colgan} and D. {Das} and A. {Ganesh} and M. {Gleeson} and S. {Hase} and A. {Holloway} and J. {Kamp} and T. {Lee} and J. {Loaiza} and N. {Macnaughton} and V. {Marwah} and N. {Mukherjee} and A. {Mullick} and S. {Muthulingam} and V. {Raja} and M. {Roth} and E. {Soylemez} and M. {Zait}},
booktitle={2015 IEEE 31st International Conference on Data Engineering},
title={Oracle Database In-Memory: A dual format in-memory database},
year={2015},
volume={},
number={},
pages={1253--1258},
keywords={data mining;database indexing;information retrieval;storage management;transaction processing;transactional consistency;analytic operation;column format;data access;index;OLTP workload;row format;dual format in-memory database;Oracle database in-memory;Indexes;Memory management;Buffer storage;Servers;Optimization;Acceleration},
doi={10.1109/ICDE.2015.7113373},
ISSN={2375-026X},
month={April},}

@inproceedings{fan2014cuckoo,
author = {Fan, Bin and Andersen, Dave G. and Kaminsky, Michael and Mitzenmacher, Michael D.},
title = {Cuckoo Filter: Practically Better Than {B}loom},
year = {2014},
isbn = {9781450332798},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2674005.2674994},
doi = {10.1145/2674005.2674994},
booktitle = {Proceedings of the 10th ACM International on Conference on Emerging Networking Experiments and Technologies},
pages = {75--88},
numpages = {14},
keywords = {bloom filters, compression, cuckoo hashing},
location = {Sydney, Australia},
series = {CoNEXT'14}
}

@inproceedings{zhu2017looking,
  author    = {Jianqiao Zhu and
Navneet Potti and
Saket Saurabh and
Jignesh M. Patel},
title     = {Looking Ahead Makes Query Plans Robust},
journal   = {{PVLDB}},
volume    = {10},
number    = {8},
pages     = {889--900},
year      = {2017},
doi       = {10.14778/3090163.3090167},
timestamp = {Tue, 16 Oct 2018 15:34:44 +0200},
biburl    = {https://dblp.org/rec/bib/journals/pvldb/ZhuPSP17},
bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Soliman:2014:OMQ:2588555.2595637,
author = {Soliman, Mohamed A. and Antova, Lyublena and Raghavan, Venkatesh and El-Helw, Amr and Gu, Zhongxian and Shen, Entong and Caragea, George C. and Garcia-Alvarado, Carlos and Rahman, Foyzur and Petropoulos, Michalis and et al.},
title = {Orca: A Modular Query Optimizer Architecture for Big Data},
year = {2014},
isbn = {9781450323765},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2588555.2595637},
doi = {10.1145/2588555.2595637},
booktitle = {Proceedings of the 2014 ACM SIGMOD International Conference on Management of Data},
pages = {337--348},
numpages = {12},
keywords = {query optimization, mpp, parallel processing, cost model},
location = {Snowbird, Utah, USA},
series = {SIGMOD'14}
}


@inproceedings{graefe1995cascades,
	title={The {C}ascades framework for query optimization},
	author={Graefe, Goetz},
	journal={IEEE Data Eng. Bull.},
	volume={18},
	number={3},
	pages={19--29},
	year={1995}
}

@inproceedings{Antova:2014:OQO:2588555.2595640,
author = {Antova, Lyublena and El-Helw, Amr and Soliman, Mohamed A. and Gu, Zhongxian and Petropoulos, Michalis and Waas, Florian},
title = {Optimizing Queries over Partitioned Tables in MPP Systems},
year = {2014},
isbn = {9781450323765},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2588555.2595640},
doi = {10.1145/2588555.2595640},
booktitle = {Proceedings of the 2014 ACM SIGMOD International Conference on Management of Data},
pages = {373--384},
numpages = {12},
keywords = {partitioning, mpp systems, query optimization},
location = {Snowbird, Utah, USA},
series = {SIGMOD'14}
}



@inproceedings{moerkotte2006analysis,
  author    = {Guido Moerkotte and
Thomas Neumann},
title     = {Analysis of Two Existing and One New Dynamic Programming Algorithm
for the Generation of Optimal Bushy Join Trees without Cross Products},
booktitle = {Proceedings of the 32nd International Conference on Very Large Data
Bases, Seoul, Korea, September 12-15, 2006},
pages     = {930--941},
publisher = {{ACM}},
year      = {2006},
url       = {http://dl.acm.org/citation.cfm?id=1164207},
timestamp = {Thu, 30 Apr 2015 18:34:40 +0200},
biburl    = {https://dblp.org/rec/bib/conf/vldb/MoerkotteN06},
bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Neumann:2009:QSG:1559845.1559889,
author = {Neumann, Thomas},
title = {Query Simplification: Graceful Degradation for Join-Order Optimization},
year = {2009},
isbn = {9781605585512},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1559845.1559889},
doi = {10.1145/1559845.1559889},
booktitle = {Proceedings of the 2009 ACM SIGMOD International Conference on Management of Data},
pages = {403--414},
numpages = {12},
keywords = {query optimization, complex joins, hypergraphs},
location = {Providence, Rhode Island, USA},
series = {SIGMOD'09}
}


@inproceedings{fender2012effective,
author={P. {Fender} and G. {Moerkotte} and T. {Neumann} and V. {Leis}},
booktitle={2012 IEEE 28th International Conference on Data Engineering},
title={Effective and Robust Pruning for Top-Down Join Enumeration Algorithms},
year={2012},
volume={},
number={},
pages={414--425},
keywords={database management systems;optimisation;query processing;tree searching;top-down join enumeration algorithms;robust pruning;optimal execution order;cost-based query optimizers;bottom-up join enumeration;optimization strategies;branch-and-bound pruning;DBMS;Partitioning algorithms;Heuristic algorithms;Robustness;Prediction algorithms;Optimization;Upper bound;Complexity theory},
doi={10.1109/ICDE.2012.27},
ISSN={1063-6382},
month={April},}

@inproceedings{astrahan1976system,
author = {Astrahan, M. M. and Blasgen, M. W. and Chamberlin, D. D. and Eswaran, K. P. and Gray, J. N. and Griffiths, P. P. and King, W. F. and Lorie, R. A. and McJones, P. R. and Mehl, J. W. and et al.},
title = {System R: Relational Approach to Database Management},
year = {1976},
issue_date = {June 1976},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {1},
number = {2},
issn = {0362-5915},
url = {https://doi.org/10.1145/320455.320457},
doi = {10.1145/320455.320457},
journal = {ACM Trans. Database Syst.},
month = jun,
pages = {97--137},
numpages = {41},
keywords = {index structures, recovery, database, nonprocedural language, authorization, relational model, locking, data structures}
}

@inproceedings{moerkotte2008dynamic,
author = {Moerkotte, Guido and Neumann, Thomas},
title = {Dynamic Programming Strikes Back},
year = {2008},
isbn = {9781605581026},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1376616.1376672},
doi = {10.1145/1376616.1376672},
booktitle = {Proceedings of the 2008 ACM SIGMOD International Conference on Management of Data},
pages = {539--552},
numpages = {14},
keywords = {complex joins, hypergraphs, query optimization},
location = {Vancouver, Canada},
series = {SIGMOD'08}
}


@inproceedings{graefe1993volcano,
author={G. {Graefe} and W. J. {McKenna}},
booktitle={Proceedings of IEEE 9th International Conference on Data Engineering},
title={The Volcano optimizer generator: extensibility and efficient search},
year={1993},
volume={},
number={},
pages={209-218},
keywords={query processing;object-oriented databases;natural sciences computing;data structures;database management systems;dynamic programming;search problems;sorting;query processing;object-oriented DBMS;Volcano optimizer generator;extensibility;efficient search;request processing;scientific database systems;logical algebra;physical algebra;optimization rules;optimizer source code;EXODUS optimizer generator;search engine;cost models;sorting order;dynamic programming;goal-directed searching;branch-and-bound pruning;rule-based optimization systems;data model independence;Volcanoes;Data models;Algebra;Power generation;Database systems;Prototypes;Search engines;Costs;Object oriented modeling;Power system modeling},
doi={10.1109/ICDE.1993.344061},
ISSN={null},
month={April},}

@inproceedings{ono1990measuring,
  author    = {Kiyoshi Ono and
Guy M. Lohman},
title     = {Measuring the Complexity of Join Enumeration in Query Optimization},
booktitle = {16th International Conference on Very Large Data Bases, August 13-16,
1990, Brisbane, Queensland, Australia, Proceedings},
pages     = {314--325},
publisher = {Morgan Kaufmann},
year      = {1990},
timestamp = {Wed, 29 Mar 2017 16:45:24 +0200},
biburl    = {https://dblp.org/rec/bib/conf/vldb/OnoL90},
bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Simmen:1996:FTO:235968.233320,
author = {Simmen, David and Shekita, Eugene and Malkemus, Timothy},
title = {Fundamental Techniques for Order Optimization},
year = {1996},
isbn = {0897917944},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/233269.233320},
doi = {10.1145/233269.233320},
booktitle = {Proceedings of the 1996 ACM SIGMOD International Conference on Management of Data},
pages = {57--67},
numpages = {11},
location = {Montreal, Quebec, Canada},
series = {SIGMOD'96}
}



==> searchalgorithm.tex <==
\section{Search Algorithm}

\subsection{Right deep tree without cross product for acyclic join graph}
\todo{Prove this is doable}


